Grain boundary slip transfer classification and metric selection with artificial neural networks

An artificial neural network is used to evaluate the effectiveness of six metrics and their combinations to assess whether slip transfers across grain boundaries in coarse-grained oligocrystalline Al foils \citep{Bieler_etal2019_2,Alizadeh_etal2020}. This approach extends the one- or two-dimensional projections formerly applied to analyze slip transfer. The accuracy of this binary classification reaches around \pcnt{87} for the best single metric and around \pcnt{90} when considering two or more metrics simultaneously. The results suggest slip transfer mostly depends on the geometric relationship between grains. Training a double-layer network having \num{10} nodes per hidden layer with \num{40} measurements is sufficient to render the maximum accuracy.

==> config.tex <==
\usepackage{etoolbox}
\usepackage{lineno}
\usepackage{xspace} % to get the spacing after macros right  
\usepackage[dvipsnames]{xcolor}
\usepackage{amsmath,amsfonts,amssymb}
\usepackage{mathtools}
\usepackage{bm}
\usepackage{siunitx}
\usepackage{textcomp}
\sisetup{exponent-product = \cdot, 
			retain-explicit-plus = true}
\usepackage{miller}
\usepackage{tikz}
\usetikzlibrary{trees,matrix}
\usepackage{forest}
\usetikzlibrary{arrows,shapes,calc,positioning}
%\usepackage[final]{showkeys} % for showing the labels in the margin
\usepackage{subfig}
\usepackage{subeqnarray}
\usepackage{multirow}
\usepackage{tabularx}
\usepackage{booktabs}
\usepackage{diagbox} % for diagonal lines in tables
\usepackage{graphbox}
\usepackage{overpic} % for superimposing images
\usepackage{enumitem} % for changing lists (especially the vertical spacing)
\usepackage{calc}
\usepackage{todonotes}
\usepackage{hyperref}
\hypersetup{
     colorlinks   = true,
     citecolor    = gray
}
\usepackage[capitalize]{cleveref}
\usepackage{doi}
%\usepackage{natbib}
\graphicspath{{./figures/}{../figures/}}
\DeclareGraphicsExtensions{.pdf,.png}

\setcounter{topnumber}{2}
\setcounter{bottomnumber}{2}
\setcounter{totalnumber}{4} 
\setcounter{dbltopnumber}{2}
\renewcommand{\topfraction}{0.9}
\renewcommand{\bottomfraction}{0.8}
\renewcommand{\dbltopfraction}{0.9}
\renewcommand{\textfraction}{0.07}
\renewcommand{\floatpagefraction}{0.7}
\renewcommand{\dblfloatpagefraction}{0.7}

% NEW COMMANDS

\newcommand{\question}[1]{\textcolor{Red}{#1?}}
\newcommand{\note}[1]{\textcolor{CornflowerBlue}{#1}}
\newcommand{\revised}[1]{\textcolor{BurntOrange}{#1}}


% ABBREVIATIONS

\newcommand{\ie}{\mbox{i.\hspace{1pt}e.}\xspace}
\newcommand{\eg}{\mbox{e.\hspace{1pt}g.}\xspace}
\newcommand{\aka}{\mbox{a.\hspace{1pt}k.\hspace{1pt}a.}\xspace}
\newcommand{\Eg}{\mbox{E.\hspace{1pt}g.}\xspace} 
\newcommand{\etc}{\mbox{etc.}}

% VARIABLES

\newcommand{\N}[1]{\ensuremath{N_\text{#1}}}
\newcommand{\Ninput}{\N{input}}
\newcommand{\Nhidden}{\N{hidden}}
\newcommand{\Ndata}{\N{data}}
\newcommand{\Ncorrect}{\N{correct}}
\newcommand{\Nwrong}{\N{wrong}}

\newcommand{\Fscore}{\(F\)-score}

% NAMES 

\newcommand{\term}[1]{#1}
\newcommand{\Eshelby}{\term{Eshelby}\xspace}
\newcommand{\Euler}{\term{Euler}\xspace}
\newcommand{\Gauss}{\term{Gauss}\xspace}
\newcommand{\KN}{\term{Kr\"oner}-\term{Nye}\xspace}
\newcommand{\PK}{\term{Piola}-\term{Kirchhoff}\xspace}
\newcommand{\Cauchy}{\term{Cauchy}\xspace}
\newcommand{\Burgers}{\term{Burgers}\xspace}
\newcommand{\NR}{\term{Newton}-\term{Raphson}\xspace}
\newcommand{\Frobenius}{\term{Frobenius}\xspace}
\newcommand{\RK}{\term{Runge}-\term{Kutta}\xspace}
\newcommand{\Orowan}{\term{Orowan}\xspace}
\newcommand{\Schmid}{\term{Schmid}\xspace}
\newcommand{\Miller}{\term{Miller}\xspace}




% PHYSICAL CONSTANTS

\newcommand{\kB}{k_\text{B}}


% CRYSTALLOGRAPHY

\newcommand{\crystaxis}[1]{\ensuremath{\langle{#1}\rangle}}

% TENSORS 

\newcommand{\field}[1]{\ensuremath{\mathbb{#1}}}
\newcommand{\tnsr}[1]{\ensuremath{\bm{#1}}}
\newcommand{\vctr}[1]{\ensuremath{\bm{#1}}}
\newcommand{\set}[1]{\ensuremath{\bm{#1}}}


% FUNCTIONS AND OPERATORS

\newcommand{\avg}[1]{\ensuremath{\overline{#1}}}
\newcommand{\norm}[2][]{\ensuremath{\left|{#2}\right|_{#1}}}
\newcommand{\pcnt}[1]{\SI{#1}{\percent}}
\newcommand{\transpose}[1]{{#1}^{\mathrm T}}
\newcommand{\inverse}[1]{{#1}^{-1}}
\newcommand{\invtranspose}[1]{{#1}^{\mathrm{-T}}}
\newcommand{\inc}[1]{\text d{#1}}
\newcommand{\sign}[1]{\operatorname{sign}{#1}}
\newcommand{\signb}[1]{\operatorname{sign}\left({#1}\right)}
\newcommand{\grad}[2][]{\operatorname{grad}_{#1}{#2}}
\newcommand{\gradb}[2][]{\operatorname{grad}_{#1}\left({#2}\right)}
\newcommand{\Grad}[2][]{\operatorname{Grad}_{#1}{#2}}
\newcommand{\Gradb}[2][]{\operatorname{Grad}_{#1}\left({#2}\right)}
\newcommand{\divergence}[1][]{\operatorname{div}{#1}}
\newcommand{\divergenceb}[1]{\operatorname{div}\left({#1}\right)}
\newcommand{\curl}[1][]{\operatorname{curl}{#1}}
\newcommand{\curlb}[1]{\operatorname{curl}\left({#1}\right)}
\newcommand{\expb}[1]{\exp{\left({#1}\right)}}
\newcommand{\partialder}[2]{\partial_{#2}{#1}}
\newcommand{\partialderb}[2]{\partial_{#2}\left({#1}\right)}
\newcommand{\partialderTwo}[3]{\partial_{#2#3}{#1}}
\newcommand{\timeder}[1]{\partial_{t}{#1}}
\newcommand{\act}{}
\newcommand{\dblCont}{:}


% SPECIAL TENSORS

\newcommand{\identity}{\tnsr I}
\newcommand{\levi}{\epsilon}


% VARIABLES

\newcommand{\SF}{\ensuremath{m}}
\newcommand{\LRB}{\ensuremath{M}}
\newcommand{\LM}{\ensuremath{m^\prime_{\alpha\beta}}}
\newcommand{\residualB}{\ensuremath{\Delta b_{\alpha\beta}}}
\newcommand{\SFsum}{\ensuremath{\text{SF}_\alpha+\text{SF}_\beta}}
\newcommand{\mproduct}{\ensuremath{\LM\,(\SFsum)}}
\newcommand{\mdivide}{\ensuremath{\log(\LM/\residualB)}}


\newcommand{\stiffness}{\ensuremath{\field C}}
\newcommand{\F}{\ensuremath{\tnsr F}}
\newcommand{\Fp}{\ensuremath{\tnsr F_\text{p}}}
\newcommand{\Fpdot}{\ensuremath{\dot{\tnsr F}_\text{p}}}
\newcommand{\Fe}{\ensuremath{\tnsr F_\text{e}}}
\newcommand{\Lp}{\ensuremath{\tnsr L_\text{p}}}
\newcommand{\E}{\ensuremath{\tnsr E}}
\newcommand{\GL}{\ensuremath{\tnsr E_\text{e}}}
\newcommand{\cauchy}{\ensuremath{\tnsrgreek \sigma}}
\newcommand{\sPK}{\ensuremath{\tnsr S}}
\newcommand{\shear}{\ensuremath{\gamma}}
\newcommand{\strain}{\ensuremath{\varepsilon}}
\newcommand{\orientation}{\ensuremath{\tnsr O}}
\newcommand{\rotation}{\ensuremath{\tnsr R}}
\newcommand{\stretchtensor}{\ensuremath{\tnsr U}}

\newcommand{\burgersvector}[1]{\ensuremath{\vctr b^{#1}}}
\newcommand{\burgerslength}{\ensuremath{b}}
\newcommand{\linedirection}[2]{\ensuremath{\vctr l^{#1}_{#2}}}
\newcommand{\slipdirection}[1]{\ensuremath{\vctr s^{#1}}}
\newcommand{\slipnormal}[1]{\ensuremath{\vctr n^{#1}}}
\newcommand{\sliptangent}[1]{\ensuremath{\vctr t^{#1}}}
\newcommand{\velocitydirection}[2]{\ensuremath{\vctr m^{#1}_{#2}}}
\newcommand{\velocityvector}[2]{\ensuremath{\vctr v^{#1}_{#2}}}
\newcommand{\velocity}[2]{\ensuremath{v^{#1}_{#2}}}

\newcommand{\shearrate}[2]{\ensuremath{\dot{\gamma}^{#1}_{#2}}}
\newcommand{\resolvedstress}[1]{\ensuremath{\tau^{#1}}}
\newcommand{\criticalstress}[1]{\ensuremath{\tau_\text{cr}^{#1}}}
\newcommand{\effectivestress}[1]{\ensuremath{\tau_\text{eff}^{#1}}}
\newcommand{\solidsolutionstrength}{\ensuremath{\tau_\text S}}
\newcommand{\attackfrequency}{\nu_\text{a}}
\newcommand{\activationvolume}[1][]{V_\text{#1}}
\newcommand{\activationenergy}[1][]{Q_\text{#1}}
\newcommand{\meanfreepath}[1][]{\lambda_\text{#1}}
\newcommand{\obstaclesize}{d}
\newcommand{\atomicconcentration}{c_\text{at}}
\newcommand{\mobility}[1]{B^{#1}}
\newcommand{\atomicvolume}{\Omega}

\newcommand{\density}[2]{\varrho^{#1}_{#2}}
\newcommand{\densitytensor}[2]{\tnsr\alpha^{#1}_{#2}}
\newcommand{\excessdensity}[2]{\varrho^{#1}_{\Delta#2}}
\newcommand{\forestdensity}[1]{\varrho^{#1}_\text f}
\newcommand{\maxdipoleheight}[2]{\hat d^{\;\!#1}_{#2}}
\newcommand{\mindipoleheight}[2]{\check d^{\;\!#1}_{#2}}
\newcommand{\edgemultiplication}{k_1}
\newcommand{\multiplicationfactor}{k_2}
\newcommand{\edgejogs}{k_3}

\newcommand{\flux}[2]{\vctr f^{#1}_{#2}}
\newcommand{\fluxdensity}[2]{f^{#1}_{#2}}
\newcommand{\interfaceflux}[2]{\widetilde{\vctr f}^{#1}_{#2}}
\newcommand{\interfacenormal}[2][]{\vctr a^{#2}_{#1}}
\newcommand{\interfacearea}[2][]{\area^{#2}_{#1}}

\newcommand{\slipsystem}{\xi}
\newcommand{\dislotype}{p}
\newcommand{\dislocharacter}{c}
\newcommand{\edge}{\text e}
\newcommand{\screw}{\text s}
\newcommand{\positive}{\ensuremath{+}}
\newcommand{\negative}{\ensuremath{-}}
\newcommand{\dipolar}{\ensuremath{\pm}}

\newcommand{\rate}[3]{{}_\text{#1}\Phi^{#2}_{#3}}
\newcommand{\jump}[3]{{}_\text{#1}\Psi^{#2}_{#3}}


% NEW UNITS 

\DeclareSIUnit\burgersunit{$\burgerslength$}
\DeclareSIUnit\micron{\micro\metre}
